Pix2Video: Video Editing using Image Diffusion

Image diffusion models, trained on massive image collections, have emerged as the most versatile image generator model in terms of quality and diversity. They support inverting real images and conditional (e.g., text) generation, making them attractive for high-quality image editing applications. We investigate how to use such pre-trained image models for text-guided video editing. The critical challenge is to achieve the target edits while still preserving the content of the source video. Our method works in two simple steps: first, we use a pre-trained structure-guided (e.g., depth) image diffusion model to perform text-guided edits on an anchor frame; then, in the key step, we progressively propagate the changes to the future frames via self-attention feature injection to adapt the core denoising step of the diffusion model. We then consolidate the changes by adjusting the latent code for the frame before continuing the process. Our approach is training-free and generalizes to a wide range of edits. We demonstrate the effectiveness of the approach by extensive experimentation and compare it against four different prior and parallel efforts (on ArXiv). We demonstrate that realistic text-guided video edits are possible, without any compute-intensive preprocessing or video-specific finetuning.

==> sections/authors.tex <==
\author{Duygu Ceylan}
\email{ceylan@adobe.com}
%\orcid{}

\affiliation{
  \institution{Adobe Research}
  \country{}
}

\author{Chun-Hao Huang}
\email{ceylan@adobe.com}
%\orcid{}

\affiliation{
  \institution{Adobe Research}
  \country{}
}

\author{Niloy J. Mitra}
\email{n.mitra@cs.ucl.ac.uk}
\orcid{0000-0002-2597-0914}

\affiliation{
  \institution{Adobe Research}
}
\affiliation{
  \institution{University College London}
  \country{}
}
 
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
% \renewcommand{\shortauthors}{Madono et al.}

==> sections/metadata.tex <==
%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
\title{
Video Editing via Consistent Residue Matching in Image Diffusion 
}

%Text-guided Consistent Video Editing via Image Diffusion Models
% Text-guided Video Editing via Consistent Residue Matching in Image Diffusion Models

\input{sections/authors.tex}

\input{sections/abstract.tex}

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{diffusion model, correspondence, text-conditioned edits}
